All Tied Up: A First Look At Modern Yo-Yo and Knot Theory

Modern Yo-Yo play has developed into a sophisticated international subculture, featuring elite competition and intricate tricks. Despite this, no systematic knot-theoretic treatment has yet been applied to the numerous string configurations realised in contemporary Yo-Yo play. This paper takes initial steps in addressing this gap, recalling fundamental results from knot theory and embeddings to develop a methodology for classifying string arrangements, known as `mounts', in both beginner and advanced single Yo-Yo play. We classify a range of mounts according to the knots they form under appropriate post-processing procedures and identify Yo-Yo maneuvers that correspond to Reidemeister moves. Furthermore, we analyse the impact of certain mounts on the writhe of their diagrammatic projections and introduce operations to facilitate discussion of composite mounts. This work seeks to initiate a dialogue between Yo-Yo practitioners and knot theorists, fostering further advancements in high-level Yo-Yo play and enabling novel physical realisations of knots, links, braids, surgeries, and other topological transformations.

==> pst-knot.tex <==
%%
%% This is file `pst-knot.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-knot.tex'
%%
%% Herbert Voss <herbert -> dante.de>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-knot' is a PSTricks package for knot macros
%%
%%
\csname PSTknotLoaded\endcsname
\let\PSTknotLoaded\endinput
% Requires PSTricks
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTXKeyLoaded\endinput\else\input pst-xkey.tex \fi
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
% interface to the `xkeyval' package
\pst@addfams{pst-knot}

\def\fileversion{0.02}
\def\filedate{2009/11/08}
\message{`PST-knot' v\fileversion, \filedate\space (hv)}
%
\SpecialCoor
\pstheader{pst-psm.pro}
%
\newdimen\psk@knot@border
\define@key[psset]{pst-knot}{knotborder}[2]{\pssetlength\psk@knot@border{#1}}
\define@key[psset]{pst-knot}{knotbgcolor}[1]{\pst@getcolor{#1}\psk@knot@bgcolor}
\define@key[psset]{pst-knot}{knotscale}[1 1]{\pst@getscale{#1}\psk@knot@scale}
\psset[pst-knot]{knotborder=5\pslinewidth,knotbgcolor=white,knotscale=1}
%
\def\psKnot{\def\pst@par{}\pst@object{psKnot}}
\def\psKnot@i(#1)#2{\expandafter\psKnot@ii(#1)#2}
\def\psKnot@ii(#1)#2-#3{%
  \addto@par{border=.5\pslinewidth}%
  \begin@ClosedObj%
  \pst@getcolor{\pslinecolor}\psk@linecolor%
  \pst@getcoor{#1}\pst@tempA%
  \addto@pscode{
    \pst@tempA\space  moveto
    tx@KnotDict begin 
    PSMinit 
    \psk@knot@scale
    \pst@number\pslinewidth SLW
    \pst@usecolor\psk@linecolor
    /knot-bgline { CLW \pst@number\psk@knot@border add SLW } def
    /knot-bgcolour { \pst@usecolor\psk@knot@bgcolor } def
    knot-#2-#3 \ifnum#2=0 \else knot \fi
    PSMclose 
    end 
  }%
  \end@ClosedObj}
%
\define@key[psset]{pst-knot}{bmcolor}{\expandafter\pst@borromean@color#1,\@nil}
\def\pst@borromean@color#1,#2,#3,\@nil{%
  \pst@getcolor{#1}\psk@borromean@colorA%
  \pst@getcolor{#2}\psk@borromean@colorB%
  \pst@getcolor{#3}\psk@borromean@colorC%
}
\psset[pst-knot]{bmcolor={red,green,blue}}
%
\def\psBorromean{\def\pst@par{}\pst@object{psBorromean}}
\def\psBorromean@i(#1)#2#3{%
%  \addbefore@par{knotborder=3}%
  \begin@ClosedObj%
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcolor{\pslinecolor}\psk@linecolor%
  \pssetlength\pst@dima{#2}%
  \pssetlength\pst@dimb{#3}%
  \addto@pscode{
    tx@KnotDict begin 
    PSMinit 
    \pst@tempA\space translate
    \psk@knot@scale
    /rgb {} def /gray {} def /cmyk {} def
    \pst@number\pslinewidth SLW
    \pst@usecolor\psk@linecolor
    /r \pst@number\pst@dima def % circle radius
    /R \pst@number\pst@dimb def % inner circle radius
    /c1 [R  90] p2r def
    /c2 [R 210] p2r def
    /c3 [R 330] p2r def
    /knot-bgline { CLW \pst@number\psk@knot@border add SLW } def
    /knot-bgcolour {\pst@usecolor\psk@knot@bgcolor} def
    /stroke-shaded {
      gsave knot-bgline knot-bgcolour stroke grestore stroke 
    } def
    c1 r circle \pst@usecolor\psk@borromean@colorA stroke 
    c2 r circle \pst@usecolor\psk@borromean@colorB stroke-shaded 
    c3 r circle \pst@usecolor\psk@borromean@colorC stroke-shaded 
    c1 r -30 30 arc \pst@usecolor\psk@borromean@colorA stroke-shaded 
    c1 r -150 -90 arc stroke-shaded
    PSMclose 
    end 
  }%
  \end@ClosedObj}
%
\catcode`\@=\PstAtCode\relax
%
%% END: pst-knot.tex
\endinput
%

